Signed iterative random forests to identify enhancer-associated transcription factor binding

Standard ChIP-seq peak calling pipelines seek to differentiate biochemically reproducible signals of individual genomic elements from background noise. However, reproducibility alone does not imply functional regulation (e.g., enhancer activation, alternative splicing). Here we present a general-purpose, interpretable machine learning method: signed iterative random forests (siRF), which we use to infer regulatory interactions among transcription factors and functional binding signatures surrounding enhancer elements in Drosophila melanogaster.

==> methods.tex <==

Traditional approaches to infer TF binding events evaluate factors independently of one another\cite{li2011measuring}. However, extensive work in enhancer biology has highlighted the importance of considering integrated, combinatorial TF interactions in relation to enhancer activity (for a review see \cite{spitz2012transcription}). Toward this end, we propose a two-stage approach to detect functional TF peaks associated with enhancer activity. First, we search for TF binding signatures, or interactions, that appear frequently across the genome. This first phase substantially reduces the set of $O(p^s)$ possible order-$s$ interactions among $p$ factors, making it computationally tractable to map putative interactions across the genome. We refer to this first phase as \textit{interaction discovery}. Next, we conduct a genome-wide scan to identify genomic regions where TF binding patterns closely resemble signatures identified in the interaction discovery phase. We refer to this second phase as \textit{interaction localization}.

\subsection*{Interaction discovery through siRF}
Data driven discovery of TF binding signatures at enhancer elements amounts to learning relationships of the form ``TF1, TF3 are unusually enriched and TF2, TF4 are unusually depleted in many known enhancer locations.'' We encode such relationships using a new mathematical notion of \textit{signed interactions}, extracted from decision tree ensembles, which represent the previous statement as $\{+1, -2, +3, -4\}$ (where $+/-$ indicate enrichment/depletion and values TF indices). Signed interactions allow us to formally address two important aspects of the statement above: (i) what constitutes unusual enrichment or depletion of a TF? (ii) which signed interactions are active at genomic regions of interest (e.g. many known enhancer locations)?

We detect signed interactions through a supervised learning framework. Consider data $\{ (y_i, \mathbf{x}_i)\}_{i=1}^n$ on genomic segments $i=1,\dots, n$, where the label $y_i \in \{0, 1\}$ denotes whether the $i^{th}$ segment is an active enhancer or not, and the feature vector $\mathbf{x}_i = (x_{i1}, \ldots, x_{ip}) \in \mathbb{R}^p$ denotes continuous measurements (ChIP-chip or ChIP-seq) on $p$ different TFs. An ensemble of decision trees (e.g. an RF) can be viewed as a collection of decision rules, each corresponding to a single leaf node in a single tree, of the form
$$
\mbox{if $x_1 > t_1, \, x_2 < t_2, \ldots, x_k > t_k$, then $y = 1$}.
$$
iRF\cite{basu2018iterative} encodes such a rule in the form of an \textit{unsigned interaction} $\{1, 2, \ldots, k \}$, representing the combination of factors that appear together in the rule. To encourage more stable use of unsigned interactions on RF decision paths, iRF iteratively re-weights feature selection to favor features that are deemed important — as defined by mean decrease in impurity (MDI) in the previous iteration.  It then uses random intersection trees (RIT) \cite{shah2014random} to search the space of rules in a weighted RF for frequently occurring unsigned interactions associated with enhancers (i.e. $y = 1$). 

In siRF, we refine this search to distinguish between TF enrichment and depletion. Specifically, we re-define the unsigned interaction above as the signed interaction $\{+1, -2, \ldots, +k \}$, representing both selected features and the direction of their associated inequalities. For every observation $i$, we generate $T$ (number of trees in the forest) encodings of the form
$$
(S_{i_t}, Z_{i_t}),\,  t = 1, \ldots, T,
$$
where $S_{i_t} \subseteq \{ \pm 1, \pm 2, \ldots, \pm p \}$ represents the signed interaction associated with the leaf node in tree $t$ which contains observation $i$, and $Z_{i_t} \in \{0, 1\}$ contains the prediction of that leaf node (see SI Appendix). This can be interpreted as a list of putative interactions, offered by $T$ different ``experts'' (trees in a forest), which explain the TF binding signatures at genome location $i$ that lead to predicted enhancer status $Z_{i_t}$. As in iRF, we use RIT to search for frequently occurring signed interactions from the space of all $nT$ encodings. We call the resulting algorithm signed iRF (siRF).

\subsubsection*{Interaction discovery through stable and predictive importance metrics}
We quantify the strength of signed interactions based on their stability and predictive power through two importance metrics: prevalence and precision. For each metric, we define a null model to quantify its behavior relative to well-known properties of TF interactions. Together, our proposed metrics and their associated null models form the basis of a predictability, computability, and stability (PCS) hypothesis testing framework\cite{yu2019three} to identify predictive and stable signed interactions. The PCS framework uses predictability to evaluate the empirical evidence for a model, computational strategies to simulate realistic reference/null distributions, and stability to assess the reproducibility of findings.

\textbf{Prevalence describes the stability of a signed interaction along decision paths.} We define the \textit{prevalence} of a signed interaction $S$ for a class $C\in\{0,1\}$ relative to a fitted RF as
\begin{equation}
  P(S|C) := \frac{1}{T}\cdot
  \sum_{t=1}^{T}
  \frac{\sum_{i=1}^{n} 
      \mathds{1}(S\subseteq S_{i_t}) \cdot 
      \mathds{1}(y_{i} = C)}
    {\sum_{i=1}^{n} \mathds{1}(y_{i} = C)}.
\label{eq:prevalence}
\end{equation}
Prevalence indicates the proportion of class-$C$ observations for which an interaction $S$ is used in predictions from the fitted RF. When an RF achieves accurate prediction, prevalence may be of particular interest as it measures the contribution of a particular interaction (i.e. proportion of decision paths where the interaction appears) on model predictions (SI Appendix, Fig. S2).

\textbf{Feature selection dependence ($FSD$)}: Cooperative binding among TFs leads to nonlinear relationships between TF concentration and binding affinity and plays an important role in producing ``switch-like'' effects that typify enhancers \cite{spitz2012transcription}. From a biological perspective, it is therefore valuable to identify TFs whose binding patterns depend on the presence/absence of other TFs. We evaluate such dependencies through feature (i.e. TF) co-occurance rates along RF decision paths relative to the null hypothesis
\begin{equation}
  H_0^{(FSD)} : P(S|C) = \prod_{s\in S} P(s|C).
  \label{eq:h0fsd}
\end{equation}
Intuitively, equation \eqref{eq:h0fsd} states that the individual features in a signed interaction appear independently of one another along decision paths of a fitted RF (SI Appendix, Fig. S3). In the context of enhancer prediction, $H_0^{(FSD)}$ states that the presence of a given TF in $S$ does not depend on the presence/absence of other TFs in $S$. To quantify deviation from this null hypothesis, we define the \textit{feature selection dependence} ($FSD$):
\begin{equation}
  FSD(S;C) := \log{\left(\frac{P(S|C)}{\prod_{s\in S} P(s|C)}\right)}
  \label{eq:intstr}.
\end{equation}
Equation \eqref{eq:intstr} compares the prevalence of a signed interaction $S$ with its expected prevalence if features were selected independently of one another. In a broad range of simulations (3 Boolean models defined over both simulated and real data), we find that filtering interactions based on $FSD$ helps differentiate between additive and non-additive components of a generative model (SI Appendix, SI Fig. S9).


\textbf{Precision describes how accurately a signed interaction predicts enhancer activity.} We define the \textit{precision} of a signed interaction $S$ for a class $C$ relative to a fitted RF as
\begin{equation}
  P(C|S) := \frac{1}{T}\cdot
  \sum_{t=1}^{T}
  \frac{\sum_{i=1}^{n} \mathds{1}(S\subseteq S_{i_t}) \cdot \mathds{1}(y_i = C)} 
    {\sum_{i=1}^{n} \mathds{1}(S\subseteq S_{i_t})},
\label{eq:accuracy}
\end{equation}
where $S_{i_t}$ is the signed interaction associated with the leaf node in tree $t$ containing observation $i$. Precision measures the average proportion of observations that belong to a given class among leaf nodes in a RF (i.e. decision paths) that contain a signed interaction $S$. When data are heterogeneous, precision can highlight signed interactions that achieve accurate prediction for select subpopulations, even if the full RF is a weak predictor across the full dataset (SI Appendix, Fig. S2).

\textbf{Minimum increase in precision ($MIP$)}: 
TFs bind many inactive regions in the genome \cite{li2008transcription}, suggesting that binding alone is not indicative of functional regulation. To distinguish putative interactions where all TFs play a functional role from those where some subset of TFs are binding in a non-functional manner, we define a hypothesis testing framework that quantifies functional/non-functional binding relative to changes in prediction accuracy. Specifically, we define the null hypothesis

\begin{equation}
  H^{(MIP)}_0 : P(C|S) = \max_{S'\subset S} P(C|S'),
  \label{eq:accdiff}
\end{equation}
which states that for a putative interaction $S$, there is some $S' \subset S$ (i.e. $S' \neq S$) that achieves comparable precision. In the case of enhancer prediction, this hypothesis states that only a subset of the TF binding events implied by $S$ are required to predict enhancer activity at the observed level of precision. To quantify deviation from this null hypothesis, we define the \textit{minimum increase in precision} ($MIP$) as


\begin{equation}
  MIP(S;C) := \min_{S'\subset S: |S'| = |S| - 1}  \log{\left(\frac{P(C|S)}{P(C|S')}\right)},
  \label{eq:accdiff}
\end{equation}
Equation \eqref{eq:accdiff} compares the precision of a signed interaction to
that of its most precise subset (SI Appendix, Fig S3). Note, in equation \eqref{eq:accdiff} we restrict ourselves to subsets $S'$ with one fewer element than $S$ to avoid an exponential increase in the number of terms that must be evaluated. Smaller subsets generally achieve comparable or worse precision than those considered in \eqref{eq:accdiff} since predictions leverage information from fewer features. In simulation studies, we find that filtering based on MIP removes interactions that include both ``active'' features (i.e. those used to generate a response) and ``inactive'' noise features (SI Appendix, SI Fig. S9).

\subsubsection*{PCS hypothesis testing to select candidate TF interactions}\label{sec:filt}
We select candidates for interaction localization by applying the recently proposed PCS hypothesis testing framework \cite{yu2019three} to the metrics defined above. Briefly, we generate a set of candidate interactions from siRF trained on the full set of training samples. We then train a collection of $B=50$ siRFs on an ``outer layer'' of bootstrap samples from the training set. Each bootstrap sample provides an estimate of MIP and FSD for each interaction, with values $< 0$ implying that the null model is more predictive/stable. We remove interactions interactions where either (i) $MIP < 0$ in more than 50\% of bootstrap replicates (ii) $FSD < 0$ in more than 50\% of bootstrap replicates (iii) the interaction is detected (i.e. returned by RIT) in less than 50\% of bootstrap replicates (i.e. stability score screening\cite{basu2018iterative}) or (iv) putatively interacting TFs are not expressed in overlapping temporal windows, as measured from an independent RNA-seq timecourse dataset (SI Appendix).

\subsection*{Interaction localization through rule-based predictions derived from siRF}
\label{sec:prediction}
The interaction discovery process described above generates a set of candidate interactions. Here, we seek to identify genomic regions where TF binding patterns resemble putative interactions. Toward this end, we decompose RF decision rules into ``modules'' associated with signed interactions. Each module represents a predictive model, which we refer to as  a \textit{localized interaction prediction}, that measures the degree to which TF binding patterns at new genomic segments resemble the pattern implied by a signed interaction. 

Consider a RF, or variant thereof, with $T$ decision trees and leaf nodes $l=1,\dots,L$. Each leaf node $l$ is associated with (i) a class label $Z_l\in \{0,1\}$ and (ii) a region of the feature space $\mathcal{R}_l=(R_1, \dots, R_p)\subseteq\mathbb{R} ^ p$ with corresponding signed interaction $S_l$. The RF prediction $\hat{y}(\mathbf{x})$ for an observation $\mathbf{x}\in\mathbb{R} ^p$ can be written as

\begin{equation}
\hat{y}(\mathbf{x}) = \frac{1}{T} \sum_{l = 1} ^ L Z_l \cdot r(\mathbf{x}, \mathcal{R}_l, S_l), \;\;\mbox{where} \hspace{1em} r(\mathbf{x};\mathcal{R}, S) := \prod_{j \in \{|k|:k\in S\}} \mathds{1}(x_j \in R_j), 
\label{eq:rfruleprediction}
\end{equation}
and $|\cdot|$ denotes absolute value. We note that the denominator $T$ comes from the fact that each observation $\mathbf{x}$ is active in exactly one rule (i.e. falls in exactly one leaf node) per tree.

\iffalse
where
\begin{equation}
r(\mathbf{x};\mathcal{R}, S) := \prod_{j \in \{|k|:k\in S\}} \mathds{1}(x_j \in R_j).
\label{eq:resp_surface2}
\end{equation}
\fi

Localized interaction predictions modify \eqref{eq:rfruleprediction} to define the RF prediction associated with a signed interaction $S$ as

\begin{equation}
\hat{y}(\mathbf{x};S) = \frac{1}{|\{l:S\subseteq S_l\}|} \sum_{l:S\subseteq S_l} Z_l \cdot r(\mathbf{x}, \mathcal{R}_l, S).
\label{eq:sirfprediction}
\end{equation}
There are two key differences between \eqref{eq:rfruleprediction} and \eqref{eq:sirfprediction}. First, \eqref{eq:sirfprediction} takes an average over leaf nodes containing a signed interaction while \eqref{eq:rfruleprediction} averages over all leaf nodes in an RF. Second, \eqref{eq:sirfprediction} is restricted to the portion of the decision rule corresponding to $S$. As a result, \eqref{eq:sirfprediction} represents an average over rules $r$ that all represent similar thresholding behavior. Predictions of this form can be viewed as a decision rule with smooth decision boundaries, defined over the features in $S$.

Such predictions exhibit several desirable properties. For instance, smooth decision boundaries make predictions less sensitive to small   changes in $\mathbf{x}$ compared with a single decision rule defined over the   same features. In addition, predictions incorporate non-linear feature interactions in the form of rules as in equation \eqref{eq:rfruleprediction}. These rules depend solely on the set of interacting features   $\{|j|:j\in S\}$.  Finally, rules in \eqref{eq:sirfprediction} define an identical functional relationship with the response of interest (e.g. enhancer activity), which can be summarized and interpreted through $S$.
